PN2SC Case Study: An EMF-IncQuery solution

The paper presents a solution for the Petri-Net to Statecharts case study of the Transformation Tool Contest 2013, using EMF-IncQuery and Xtend for implementing the model transformation.

==> eptcsdata.tex <==
\providecommand{\firstpage}{106}
\providecommand{\publicationstatus}{Pieter Van Gorp, Louis M. Rose, Christian Krause (Eds.):\\
Sixth Transformation Tool Contest (TTC 2013)\\
EPTCS 135, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.135.14}{10.4204/EPTCS.135.14}}
\pdfoutput=1

